Machine Explanations and Human Understanding

Explanations are hypothesized to improve human understanding of machine learning models and achieve a variety of desirable outcomes, ranging from model debugging to enhancing human decision making. However, empirical studies have found mixed and even negative results. An open question, therefore, is under what conditions explanations can improve human understanding and in what way. Using adapted causal diagrams, we provide a formal characterization of the interplay between machine explanations and human understanding, and show how human intuitions play a central role in enabling human understanding. Specifically, we identify three core concepts of interest that cover all existing quantitative measures of understanding in the context of human-AI decision making: task decision boundary, model decision boundary, and model error. Our key result is that without assumptions about task-specific intuitions, explanations may potentially improve human understanding of model decision boundary, but they cannot improve human understanding of task decision boundary or model error. To achieve complementary human-AI performance, we articulate possible ways on how explanations need to work with human intuitions. For instance, human intuitions about the relevance of features (e.g., education is more important than age in predicting a person's income) can be critical in detecting model error. We validate the importance of human intuitions in shaping the outcome of machine explanations with empirical human-subject studies. Overall, our work provides a general framework along with actionable implications for future algorithmic development and empirical experiments of machine explanations.

==> concept_definitions.tex <==

\section{A Theoretical Framework of Human Understanding}
\label{sec:framework}

We build a theoretical framework of human understanding using the aforementioned concepts as pillars.

\subsection{Formalizing Three Concepts of Interest}
\label{sec:three_measures}

\shi{subsection title is redundant}

\shi{The following is still a repetition of Section 2.}

Generally speaking, we are interested in systems that consist of a task, a model, and a human.
We think of \taskboundary, \decisionboundary, and \errorboundary as theoretical constructs that only depend on the first two parts (task and model), but not the human.
This is to be distinguished from the \textit{human understanding} of these concepts, which we will discuss later.

\begin{itemize}
\item \textbf{\Taskboundary} is the function $f: \inputspace \rightarrow \outputspace$ that represents the groundtruth mapping from input to output.
\item \textbf{\Decisionboundary} is another function with the same domain and range $g: \inputspace \rightarrow \outputspace$ that represents our machine learning model.
Models are often not perfect, and they make mistakes in some areas of the input space.
\item \textbf{\Errorboundary} as a third function $u: \inputspace \rightarrow [0, 1]$, an indicator of whether the model prediction is correct; in other words $u(X) = 1[f(X) == g(X)], \forall X \in \inputspace$.
\end{itemize}

Figure~\ref{fig:base_diagram} visualizes the relationship between $X$, $Y$, $\hat{Y}$, and $U$.
We also use functions $f,g$, and $u$ to label the edges.

We do not assume that these theoretical constructs to be realizable: if $\inputspace$ corresponds to all possible program---input pairs, an algorithm $f$ to predict whether the given program will halt on the input does not exist. \chacha{i dont understand this paragraph}
We are, however, interested in whether these functions are ``realizable'' by a human\footnote{Abuse of term.}, which we discuss later in the section.

























==> current_state.tex <==







\subsection{Current State of Machine Explanations}




\begin{table*}[htbp]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.2\linewidth}p{0.4\linewidth}p{0.38\linewidth}}\toprule
       Machine explanation & Definition & Examples \\\hline\hline
       Local \textbf{feature} importance & Given a single data example, quantify each feature’s contribution to the prediction. & Wizard of Oz \citet{binns2018s,bussone2015role,buccinca2021trust,buccinca2020proxy}, SHAP \citet{weerts2019human,kaur2020interpreting,zhang2020effect,zhang2019dissonance}, coefficients \citet{wang2021explanations,green2019principles,kaur2020interpreting,nguyen2018comparing,hohman2019gamut,smithrenner2020,lai2020chicago,feng2018can,dodge2019explaining,ghai2020explainable,lai2019human}, tree-based/rule-based explanation \citet{kulesza2013too,lakkaraju2016interpretable}, attention \citet{lai2020chicago,chandrasekaran2018explanations}, saliency \citet{nguyen2018comparing}, LIME \citet{nguyen2018comparing}, inline highlights \citet{bansal2020does}\\
        Global \textbf{feature} importance & Overall importance of different features in influencing model predictions. & SHAP \citet{kaur2020interpreting,zhang2020effect}, coefficients \citet{dodge2019explaining}, permutation-based \citet{wang2021explanations}  , shape function of GAMs \citet{hohman2019gamut}, Wizard of Oz \citet{binns2018s} \\
        \midrule
        Nearest neighbor/similar \textbf{examples}   & Given a single data example, find examples with similar features, predictions, or both. & \citet{cai2019human,binns2018s,cai2019effects,kulesza2013too,kunkel2019let,buccinca2020proxy,wang2021explanations,hohman2019gamut,dodge2019explaining,lai2019human} \\
       Representative \textbf{examples} & Pinpoint one or a set of training samples that deem to be representative or important to a certain prediction output. &  \citet{cai2019effects,feng2018can,lai2020chicago} \\
        Counterfactual \textbf{examples}  & Given a single data example, ask ``what-if" questions to observe the effect that modified features have on its prediction. & Counterfactual~\citet{friedler2019assessing,binns2018s,wang2021explanations,hohman2019gamut,dodge2019explaining,10.1145/3442188.3445917}, contrastive~\citet{lucic2020does}\\
       \midrule
              Inherent interpretable \textbf{models} &  Showing the internal structures and all the parameters of the model. &  \citet{poursabzi2018manipulating,friedler2019assessing,lakkaraju2016interpretable}
              \chacha{add model type here }\\

        \bottomrule
    \end{tabular}}
    \caption{Ingredients of machine explanations. The targets of different explanations are in bold.\chacha{table 2 updated, i deleted error boundary related explanations}}
    \label{tab:explanations}
\end{table*}




We start by reviewing typical ways machine explanations are generated. 
Machine explanations are generated to unravel the underlying mechanisms behind a model, and can be grouped into three categories: feature-based explanations, example-based explanations, and inherent interpretable models.
We present a detailed view of different explanation methods with definitions along with citations of papers that use such explanations when evaluating human understanding in Table~\ref{tab:explanations}.

\chenhao{maybe we should stay with local explanations.}
\chacha{according to table 2, global feature importance and inherent interpretable models are global explanations, others are all local explanations.} 

 


\para{ \textbf{Feature-based explanations}}, including local feature importance and global feature importance, are commonly used explanation methods. Local feature importance quantifies each feature's contribution (or importance) to a given prediction, while global feature importance quantifies the feature importance to the overall model. 
For example, when predicting property values, certain features are more important to the overall prediction (e.g., lot size and number of rooms) while others might be less important (e.g., distance to a school). When predicting a certain house value, some feature might stand out (e.g., the house has 2 parking spaces and are convenient to a good local school), while others might not affect the prediction much (e.g., average lot size).
    
\para{ \textbf{Example-based explanations}}, including nearest neighbors, representative examples, and counterfactual examples, are another major category of explanation methods. Those methods explain in the form of sample inputs (or instances). 
One common example-based explanation technique, the nearest neighbors, is to showcase instances from training dataset that are similar to the given input. As these examples come from the training dataset, they are labeled with the ground truth prediction. 
For example, we might explain the predicted price for a given home by showing similar homes with their actual prices. 
Another example-based explanation technique is to pinpoint one or a set of training samples that are representative of or important to a certain prediction output~\citet{nguyen2016synthesizing}. 
Alternatively, counterfactual explanations provide hypothetical examples with minimal changes to the original feature values that would result in a different pre-defined output, in other words, counterfactual explanations provide ``what-if'' instances for a different model outcome.
For example, a counterfactual explanation for loan prediction task could be ``you would have received the loan if your income was higher by \$10,000.''
    
\para{\textbf{Inherent interpretable models}}, different from the aforementioned two types of post-hoc explanations, are built-in explanations inherently from the model itself. Those models are inherently explainable by design, most of which have simple structures, such as decision trees, decision sets, or sparse linear models. Some works visualize the whole model with their parameters to users to measure their understanding.


\subsection{Relationship between $E$ and the model}
or types of machine explanations
\chacha{We'll come up with a better subsec title}


\para{Proximal mechanism vs. evidence}. To better understand the effect of machine explanations and how they help with human understanding, what kind of information they convey. We further group them into two categories of interest: proximal mechanism and evidence, based on the information they convey, following some psychology works \citet{lombrozo2006structure}. Proximal mechanism explains the mechanism between how an input is mapped into a label, while on the contrary, evidence does not provide any information on \textit{how} explanations leads to the model. For example, in sentimental analysis where in a given paragraph, if the explanation only contains highlighted tokens which are relevant to the prediction, the explanation is deemed as evidence; if the explanation contained highlighted tokens associated to different sentiments (positive and negative), the explanation is proximal mechanism. 
\chacha{mechanism conveys U or not, and why? probably mechanism + human intuition lead to U}

\chacha{Attention or unsigned weights are evidence}

\chenhao{are we going to have partial decision boundary as a thing?}
\chacha{partial decision boundary belong to mechanism?}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/evidence_vs_mechanism.pdf}
    \caption{An example of evidence vs. mechanism. \chacha{as an illustration, refine later}}
    \label{fig:my_label}
\end{figure}




\para{Correlation between $E$, $Y$, and $\hat{Y}$}.
Previously we reviewed current state-of-the-art explanation methods, In this section, we focus on what information do explanations convey. 
In the local instance level, machine explanations, including feature-based and example-based explanations, are generated by the machine learning model. Hence, as illustrated in \figref{fig:exp_correlation}, $E$ is directly derived from the individual machine predictions $\hat{Y}$, while $\hat{Y}$, given by the model trained on the training data, is affected by groundtruth label $Y$. With that, we conclude that $E$ is independent of $Y$ and $U$ given $\hat{Y}$. For instance, feature importance derived from the weights of a logistic regression model, is relevant to the current prediction label $\hat{Y}$, while independent of the groundtruth label $Y$ conditioned on $\hat{Y}$.


Note that other information people may provide like confidence scores can be correlated with $U$. But they are not considered as typical machine explanation methods. We leave the discussion of those methods in Appendix. \chacha{todo-appendix}


mechanism (signed feature importance)
evidence
curve/partial decision boundary


mechanism tells you the reasoning process so that is U




\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figs/explanation_role.png}
    \caption{Explanations $E$ are correlated with $\hat{Y}$. Given $\hat{Y}$, $E$ is independent of $Y$. However, in some use cases, we desire $E$ to be correlated with $Y$, or $U$.}
    \label{fig:exp_correlation}
\end{figure}



























































 






==> discrepancy.tex <==





disrepancy or superpower of human priors


\section{Implicit Role of Human Priors}
\chacha{or super power of human priors}





\begin{assumption}
When model explanations represent spurious patterns (or more generally ``wrong intuitions), humans are able to recognize them based on their priors.
\end{assumption}
\citet{buccinca2020proxy,wang2021explanations,chandrasekaran2018explanations,bussone2015role,buccinca2021trust,green2019principles,weerts2019human,zhang2020effect,lai2019human,lai2020chicago,feng2018can,bansal2020does} 

one recent example \citet{buccinca2020proxy} demonstrates

\begin{assumption}
Shallow explanations can help gain a deeper understanding, with human priors filling in the gap.\chacha{?}
\end{assumption}


\citet{buccinca2020proxy,wang2021explanations,chandrasekaran2018explanations,bussone2015role,buccinca2021trust,green2019principles,weerts2019human,zhang2020effect,lai2019human,lai2020chicago,feng2018can,bansal2020does,nguyen2018comparing,lucic2020does,poursabzi2018manipulating} 



























\subsubsection{\decisionboundary vs. Error Boundary}
It is worth noting that understanding of \decisionboundary is solely related to the model while understanding the error boundary is beyond the model. 
The direct mapping of human understanding to \decisionboundary is the simulatability, while error boundary is the human-AI performance.
Full understanding entails a $100\%$ accuracy in simulatability.

The \decisionboundary and error boundary is distinct and parallel in terms of the understanding level. One is often not derived from another. They should be measured separately. \amit{great point! I guess OOD accuracy will be a good point to add here. OOD test data points will affect error boundary but have no effect on \decisionboundary. }
\subsubsection{Navigating the Taxonomy}
We show a detailed view of each level of human understanding in Table~\ref{tab:understanding}. We also give examples of how people solicit the questions regarding each understanding level in their human subject experiments. 

\chacha{what are the observations}
The direct way to measure the human understanding of \decisionboundary is via simulatability. If a person understands the \decisionboundary perfectly, he/she will be able to simulate the model behavior. \chacha{examples examples}

Similarly, the direct way to measure human understanding of error boundary is via complementary performance. 
Error boundary is essential towards a complementary performance, in which case humans can perfectly identify the machine errors and thus making a correct decision/prediction.
\chacha{examples examples} 

Besides, researchers also evaluate other factors such as feature importance, similar examples, etc. These measurements usually are achieved by asking the participants to answer multiple-choice questions. A common way is to show directly the groundtruth answer to human subjects during the experiments. Usually, they are not generalizable and only serve as a checklist of whether the participants can utilize the shown explanations, e.g. showing all the local feature importance and asking about which features are most important.






\subsection{With Limited Explanations Comes Great Responsibility}














In \citet{feng2018can}, predictions with confidence, representative examples and important features (decision boundary) are shown to the participants, while they are tested with human-AI performance (error boundary).
We posit that in such discrepancy, human intuition/commonsense will fill in that gap. \chacha{But what else? }


\section{Implications of these Discrepancies}
\chacha{or What are missing components for humans to achieve these understandings? (or what comes in if the discrepancy exists)}

Experiments won't be able to accurately measure the intended effects.
(main argument and many ways to unfold it)




\subsection{Human intuition/domain expertise/bakcground knowledge could be zero}
These studies are about human-AI collaboration. The implicit assumption by the researchers is that humans can fill in this gap.
(Researchers are making unrealistic assumptions of human intuitions.)


Researchers are not targeting the right type of explanations.

Researchers are not using appropriate tasks.

\paragraph{Human intuition is not static}
how human update their intuition









\section{Implications for Complementary Performance}

Either change the explanation or change the question/required understanding


What are necessary ingredients towards complementary performance (human + AI $>$ AI, human +AI $>$ human)?

So far, we have been assuming perfect learners.

incentives



\section{Discrepancies between Current Explanations and Their Evaluations}

In this section, we first review the evaluation of human understanding in practice, then provide an overview of existing machine explanations methods, and show that most of them are derived from the model, hence can only convey information related to the model decision boundary. Naturally, we uncover our findings as the inherent challenges existed in human understanding, and the discrepancies with the human evaluations and their expectations.


\subsection{Machine Explanations and Their Magic Power}

\chenhao{we should probably change section titles. I think that we should discuss in this section what explanations typically show, and what they explain. }
\chacha{agree.}

The goal of machine explanations is to build human understanding. In this section, 
We first showcase that existing popular methods of machine explanations are all describing the decision boundary. In rare cases, machine explanations can be useful to error boundary. Importantly, no machine explanations can directly improve the understanding of the task boundary, which is an intermediate step towards the goal of improving the task performance. 





\para{Ingredients of machine explanations.}
We showcase common forms of explanations that have been studied in the field with descriptions and citations of papers that use such explanations when evaluating human understanding.
We gave a detailed review of different ingredients in prior works in Table~\ref{tab:explanations}. By enumerating common machine explanations methods, we argue that most of the explanations are only about the decision boundary, since they derived from the model. Explanations methods do not really investigate on the groundtruth data, but works on the model.









































\subsection{Inherent Challenges in Achieving Ideal Understandings} 

\label{sec:discrepancy}
Deep learning models are increasingly adopted because of their (perceived) superior predictive power.
These models tend to contain millions or even trillions of parameters.
Their task boundaries are thus non-linear and can be very complex for humans to understand.
We argue that these inherent challenges render it {\em impossible} for humans to {\em complete} understand complex deep learning models.


\para{Fully understanding is impossible for deep learning models/complex tasks.} Understanding the \decisionboundary requires a complete understanding of $h(\cdot)$, which consists of millions or trillions of parameters for large deep learning models. 
In order to completely understand the decision boundary of these models, humans need to store a large number of parameters and perform a gigantic amount of computation.
\chenhao{since these deep models can apply to emulation task, maybe we should not talk about all understandings here.}
Hence, it is commonly believed that it is impossible for humans to fully achieve the ideal understanding ($f(\cdot)$, $h(\cdot)$, and $u(\cdot)$) for complex deep learning models \citet{doshi2017towards,rahwan2019machine,samek2017explainable}. 









\chenhao{all explanations are intrinsincally shallow may go to 2.3, and ideal understanding is impossible can go to 2.1.2, relationships. We should move discrepacy here and start with: 1) most explanations are about decision boundary, but more evaluations are about task boundary/error boundary. 2) explanations are shallow but we expect deep behavior.}

With those gigantic deep learning models, researchers have been relying on machine explanation methods to increase the level of interpretability. However, another critical aspect arises:
\textbf{all machine learning explanations are intrinsically shallow.}
Most of the existing explanations methods are very shallow and can not fully convey the mechanism of how a model makes a prediction, let alone the faithfulness of the generated explanations.\chenhao{not sure why let alone ... the flow is a bit strange here.} Often, those methods use a single-layer neural network. Some others as two or three-level decision trees. 
\footnote{There is one exception in shallow explanations, once we theorize a deep learning model for the underlying complex patterns it learns, we would be able to provide a somewhat deep explanation, or when there exists a simple model which achieves equivalent performance with the original large deep models. }






The shallowness of the machine explanations is rarely studied in the literature in Machine Learning. \chacha{double check}
The psychology literature, on the contrary, has long studied the limits of explanations. 
\citet{wilson1998shadows} explicitly points out that explanations are shallow, due to the individual cognitive ability limitations. They define explanations as a successful attempt to increase the understanding of a phenomenon, which does not encompass the depth that we may expect. Previously, a rich line of psychology work \citet{hempel1965aspects,nagel1963structure,salmon1989four,kitcher1989explanatory} has discussed the limitations in scientific explanations, from a cognitive science perspective. The growth of explanatory power is increasing along with the articulation of theories. While in most cases, explanations are shallow and they become deep when they are transformed into scientific theories which describe the underlying phenomenon they try to explain. The progression bar with increasingly explanatory power from prediction $\rightarrow$ understanding $\rightarrow$ explanations $\rightarrow$ theories have long been debated in the psychology literature, but rarely brought into attention in ML.

\chenhao{it may be interesting to give the analogy of humans not able to give deep explanations in most cases. Need to think about it more. This could backfire since humans sometimes give deep explanations, e.g., science.}






Overall, this property of limitation is
\chenhao{not sure what this property of limitation means, just an English thing.}
largely overlooked in the existing literature, both in ML and HCI. Sometimes researchers design experiments with an unrealistic goal of fully understanding the model. It is important to clarify the inherent limitation nature in both explanation and understanding. Next, We give a detailed review of current human understanding metrics in Section~\ref{sec:evaluation_understanding} and a full categorization of machine explanations in Section~\ref{sec:explanation_ingredients}, showing how this inherent challenge manifests as discrepancies in existing work.


\amit{in addition, it may be good to categorize human explanation and  fidelity of machine explanation}







\begin{table*}[htbp]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}p{0.15\linewidth}p{0.45\linewidth}}\toprule
    Category &  Understanding level & Definition & What are the questions people ask? \\\hline
       \multirow{5}{*}{C1 \& C2}&Nearest neighbor/similar \textbf{examples}  & identify similar data samples, by feature, by label, or both  & 
           1) Given a house and its predicted price of \$250,000, what other houses have similar features, price, or both?~\citet{hohman2019gamut} \newline
           2) Given a house and a binary model prediction that says to “buy”, what is the most similar real home that the model predicts “not to buy”?~\citet{hohman2019gamut}
       \\
       &Counterfactual/contrastive \textbf{examples}  & answer ``what if'' question& 1) Given a house and its predicted price of \$250,000, how would the price change if it had an extra bedroom?~\citet{hohman2019gamut} \newline 2) Given a house and its predicted price of \$250,000, what would I have to change to increase its predicted price to \$300,000?~\citet{hohman2019gamut}\newline
       3) Ask the participants to manipulate input to change output~\citet{lucic2020does}\\
       &Local \textbf{feature} importance & identify feature importance to a specific sample & 1) Given a house and its predicted price of \$250,000, what features contributed to its price?~\citet{hohman2019gamut} \newline 2) Participants were given a reference profile, and they were asked to select from a list of changes in feature values the ones that they believed would result in an opposite model prediction~\citet{wang2021explanations}
 \\
       &Local marginal effect of \textbf{feature} & identify marginal effect to a specific sample &1) Specify a feature’s marginal effect on predictions: participants were asked questions like “if the value of feature X of this profile is x2 instead of x1, would it increase or decrease the chance for the model to predict Y ?”~\citet{wang2021explanations} \\
        &Simulatability & simulate model predictions given global samples & 1) Simulate model behavior: participants were given a profile, and they were asked to predict what the model would predict on this profile~\citet{wang2021explanations}\newline
        2) Guess what the model would predict and state their confidence (in this guess and in model's prediction)~\citet{poursabzi2018manipulating}\newline
        3) Descriptive question ask the users to describe the \decisionboundary~\citet{lakkaraju2016interpretable}
        \\\hline
       \multirow{5}{*}{C2} &Input \textbf{features} & identify used features & Participants discussed specific features used by the model~\citet{kulesza2013too} \\
        &Global \textbf{feature} importance & & 1) Compare feature importance: participants were asked to select among a list of features which one was most/least influential on the model’s overall predictions~\citet{wang2021explanations}\newline
        2) “Which is the 3rd most important feature for the underlying model, according to the explanation system?”\citet{kaur2020interpreting}
        \\  \hline

      \multirow{2}{*}{C3 \& C4}   
        & Regions of error/training \textbf{data} distribution & Given a model, locate regions of the model where prediction uncertainty is high. &  1) Given a house price prediction model trained mostly on older homes ranging from \$100,000 - \$300,000, can I trust a model’s prediction that a newly built house costs \$400,000?~\citet{hohman2019gamut}\\
        & Human-AI agreement/human-AI performance & Human performance with AI assistance or AI error detection &1) Error detection: participants were given a profile, the model’s prediction on the profile, and the model’s explanation (if applicable), and they were asked to determine whether the model’s prediction was correct~\citet{wang2021explanations}\newline
        2) Please rate your agreement with the following statement: ‘I agree with the decision’~\citet{binns2018s}\newline
        3) Participants final prediction accuracy after seeing AI information ~\citet{zhang2020effect}\newline
        4) Their own prediction and state their confidence (after revealing machine prediction)~\citet{poursabzi2018manipulating}\newline
        5) Guess whether a VQA model will answer this question for this image correctly~\citet{chandrasekaran2018explanations}\newline
        6) Complementary performance~\citet{feng2018can,bansal2020does}\newline
        7) Human-AI agreement~\citet{bussone2015role,park2019slow,buccinca2021trust}
\\
        \bottomrule
    \end{tabular}}
    \caption{Levels of human understanding. }
    \label{tab:understanding}
\end{table*}


\subsection{Discrepancies}

When the machine explanation and human understanding mis-align, it can not reflect properly to what extent the explanations help, also shown in \citet{wang2021explanations}.

\textbf{\textit{We show shallow explanations, but test on the deep understanding.}
}
We argue showing the decision boundary or showing the error boundary is the deepest way of showing explanations. A lot of the previous work demonstrate a discrepancy in showing shallow explanations but test on deep understanding. For example, by showing the feature importance, participants are tested on the simulatability. 


\textbf{\textit{We show explanations from decision boundary, but test on the error boundary.}
}
It's important to emphasize that the decision boundary and error boundary are distinct and parallel aspects of human understanding.
\chacha{what about showing feature importance-->feature importance does not make sense to human-->human think the prediction could be wrong because the model is looking at wrong features. Does that mean feature importance helps with understanding error boundary?}

\subsection{Summary}

To summarize, our work identify the following important directions:

\chenhao{we need to think about how to structure this paper, but I think that the framework will take about 5 pages and we can write 3 pages for an experiment.}




==> explanation_ct.tex <==

\section{The Role of Explanations}
\label{sec:explanations}

Our framework can help understand how explanations influence different types of human understanding.
Before the formal discussion, let's look at a case study.
The task is to detect deceptive reviews using the dataset from \citep{ott2011finding}.
The dataset contains authentic and deceptive reviews for hotels in the Chicago area, and the deceptive ones are authored by people who have never stayed at the hotel.
In this task, ML models outperform humans by a significant margin~\citet{lai2019human}, and the models do so by recognizing patterns that are unknown and counterintuitive to humans.
For example, the word ``Chicago'' turned out to be highly predictive of deception,
possibly caused by the lack of specificity when authors imagine their experience.
This pattern is valid and easily discoverable by an support vector machine (SVM) with unigram features, but most people do not have this intuition for deception detection.

Now, imagine we ask a human to assess the correctness of the SVM's predictions.
Following typical interpretable ML setup, we highlight words that the model most rely on when making predictions.
The word ``Chicago'' will be frequently highlighted for deceptive reviews for which the model prediction is correct. 
But the human would be inclined to question the model predictions for those examples, since the highlighted words---according to the human's intuition---seem irrelevant.
As a result, the human is more likely to misjudge the model prediction as incorrect, compared to not having explanations.

What went wrong?
The model correctly identified a highly predictive feature from the training data and correctly applied it to test examples; the explanation also highlighted that feature, faithfully.
But there is a gap between what the human considers relevant and what the model finds predictive.
To bridge the gap, we can try to align the model with human intuition by disallowing counterintuitive features, but we would miss out on valid patterns and sacrifice model accuracy.
Alternatively, we could try to convince the human that the association between ``Chicago'' and deception is supported by evidence, for example by visualizing how ``Chicago'' appears far more frequently in deceptive reviews than authentic ones.
Finally, we could provide a summary of the model's accuracy when different words are highlighted, in the hope that the human learns to trust the model when ``Chicago'' is highlighted.
\chenhao{I am not sure we have a good alignment with each of these. I think discussing solutions is too much before the example. I think that the case study can also come later since 4.1 does not require the example.}

Explanation plays a different role in each of these solutions.
In this section, we use causal diagrams to formalize the role of expalantions in shaping human understanding.
We also discuss where existing methods fail to fulfill these roles, and describe properties that a solution should have.
\chenhao{overall, I like this example, but it might a bit too much in the beginning. I am going to leave it as is.}

\subsection{Limitation of Machine Explanations}

The value of explanations is defined by how much they improve human understanding quality.
Under our framework, the quality of understanding is measured by the accuracy of the human approximations evaluated against the ground-truth foundation variables.
The informativeness of an explanation can thus be defined as how much it improves such accuracy, in other words difference in human approximation accuracy with and without the explanations.

We first examine the fundamental limitations of post-hoc
\chenhao{our claims are not only about post-hoc?}
explanations by asking: is it theoretically possible to construct explanations that are more informative than model predictions \chenhao{the model? It is certainly possible to construct explanations more informative than model predictions.}?
Since the explanations and predictions are derived from the same model, it is not immediately clear why the answer should be positive.
For settings where the answer is definitively negative, i.e., explanations are no more informative than model predictions, we can say that in those settings explanations add no practical value.
\shi{This is a response to the two comments above and argument for limiting to post-hoc explanation vs.\ model prediction for now. Once we start to talk about ``understanding the model'' or start to make comparisons of explanation vs.\ model itself, we will inevitably run into a circular argument that takes us nowhere. The chain of reasoning is the following: using the causal diagram we see that, given the model, explanation doesn't help. Then the question would be: what does ``given the model'' mean for humans? Without making assumptions about what ``understanding the model'' means, the only conclusion we can reach is ``if you understand the model, you don't need explanations'', which deduced without this much effort e.g., invoking the causal diagram. The next question would be: how should we define ``understanding the model''? Obviously this is a difficult question, and our current understanding on this issue is pretty much black-and-white: a model is either fully understandable or totally incomprehensible. In conclusion, if our discussion involves any notion of ``understanding the model'', we are stuck. Instead, we should discuss the informativeness of explanations without making assumptions about what ``understanding the model'' means. The most basic comparison here---which seems almost too basic---is the comparison between post-hoc explanation and model prediction itself. People take it for granted that explanations can provide value beyond what's already conveyed in model predictions, but that is not necessarily true, and we show that in this subsection. We are basically trying to say that, even for this very basic statement, assumptions about human intuition are required for it to be true. Of course this can be seen a very circular way of motivating assumptions about the ``human understanding of the model'' but I think it's useful. The next subsection talks about one possible way to formalize these assumptions.}
\shi{I just thought of another way to frame this. Using the causal diagram, we see that given the model, explanation is useless. Another way to put it is, if you want a better understanding (according to the foundation variables), you need to either understand the model or have useful explanations; the former is the approach taken by using transparent models, the later post-hoc explanations. In this section, we are trying to figure out the necessary conditions for useful post-hoc explanations.}

Among all settings listed in the decision tree (\figref{decision_tree}), it is clear that the answer would be negative for all emulation tasks.
In those settings, humans have perfect knowledge of the \taskboundary, and once provided with model predictions, humans would achieve perfect accuracy at approximating the three foundation variables, which is considered a ``perfect understanding'' in our framework.
Note that when we say that explanations have no practical value, we only mean it in the narrow sense that it cannot help human achieve better approximation than predictions.
Emulation tasks are often used as testbed for evaluating properties of explanations such as faithfulness, and we discuss these use cases later in the paper \chenhao{are we going to discuss this later? This paragraph is good though!}.
\shi{If there is enough space, one useful thing to discuss is the assumptions about transferability that people tend to make. The most common assumptions is that the faithfulness evaluation results can transfer from emulation to discovery tasks.}

The case of discovery tasks is much less obvious.
We cannot rule out the possibility of a more informative explanation, but it is unclear what it should look like.
For example, in deceptive review detection\ldots
Our next question is then: is our framework sufficient for comparing the informativeness of explanations for discovery tasks, or do we need to introduce new concepts?

\begin{figure}
    \centering
     \includegraphics[width=.45\columnwidth]{figs/explanation_independence}
    \caption{
        Instance-level local explanation $E$ is constructed for each input $X$ individually based on model parameters $\theta$.
        Conditioned on the model, the input, and model prediction which are readily available to humans, the explanation 
        \chenhao{the external information does not have to go to E?}
    }
    \label{fig:explanation_independence}
\end{figure}

We visualize how explanation interacts with the foundation varaibles in \figref{fig:explanation_independence}.
As shown in the diagram, instance-level, local explanation $E$ is constructed for each input $X$ individually based on the model $g$, so it shares the same parents as the model prediction $\yhat$.
Applying d-seperation we see that, when conditioned on the model $g$ and the input $X$, the explanation $E$ is independent of both $Y$.\footnote{Explanation $E$ is also conditionally independent of $Z$ given $g$ and $X$. In fact, a variable that is d-seperated from $Y$ is also d-seperated from $Z$; whenever $Y$ is not conditioned on, the converse is also true. To simply the discussion, we focus on conditional independence with $Y$.}
The independence implies that explanation gives us no extra information about the label once we have knowledge of the model and the input.

But this observation isn't very helpful; it is unclear what ``knowledge of the model'' means.
When we fully understand the model, explanations are useless; but when we do not have full knowledge of the model, it is not clear how to quantify that knowledge.
In other words, we can only reason about the extreme cases; the general case remains unclear.

Our point is that the extra information must come from somewhere else, which is also saying that our framework cannot capture how the extra information is communicated from the external source to the explanation.

In a discovery task, both $\humany$ and $\yhat$ are imperfect approximations of $Y$.
How can we build a better approximation of $Y$ based on $\humany$ and $\yhat$?

Conditioned on the model and the input, explanation is independent of all three foundation variables. This is just another way to say: ``if the model is fully understandable, you do not need explanations.''

But in cases where full understanding of the model is impossible, it is also unclear how to quantify human understanding.
Any improvement in the human approximation of foundation variable must come from somewhere outside the foundation variables. There must be an external source that is not yet included in our framework.
\chenhao{I see where you are going. I think that this is interesting, but it may be perceived as confusing. Let me think about it. But we are on the same page enough that you can certainly move on to the next subsection.}


\shi{So the takeaway from the above is that, even for the seemingly simple goal (and the prerequisite of including explanations in actual application) of construction explanations that are more informative than predictions, we need to make assumptions about human intuition. I think what should follow is a discussion of assumptions made by current machine explanations.}


\subsection{Explanation + Human Intuitions}

\paragraph{Explanations as task decomposition.}
Explanations can be seen as exposing intermediate steps of the model's black-box process of computing the output from the input.
Conceptually, the explanation acts as a pivot that decomposes the task into two parts, and its connections with both the input and the output are important.
The human's interpretation of these two connections is shaped by many factors: the format of the explanation, the human's prior knowledge about the task and the model, and many more.
Note that the model's underlying computation does not necessarily align with what's implied by the explanations, for example, feature attribution explanations visualized using heat maps imply that the underlying model employs a feature extraction process, but the neural model in fact always looks at the whole input.
The task decomposition implied by the explanation is not guaranteed to be faithful, and the human's interpretation of the computation process might not align with what's actually happening in the model; in other words, human interpretations are likely not be faithful.
But nonetheless, these interpretations have large influence on how human work with the model.

A broad-stroke depiction of feature attribution explanation, a broad-stroke description of is it decomposes two parts can be thought of as relevance and mechanism.
Relevance is an encoder of the input $X$ whose output is the feature attribution explanation $E$, mechanism is the decoder that maps the explanation $E$ to the output $\humany$.


\subsection{Limitation of Current Machine Explanations}

We start by introducing current commonly used machine explanations and add them to our causal diagrams.
\chenhao{explain the difference between training and inference, the fact that it is conditioned on $g$}
\chenhao{we need to define given $g$}

\paragraph{Current machine explanations.} Two common approaches to explaining machine predictions are 1) inherently interpretable models, and 2) post-hoc explanations, including feature-based approaches such as LIME and SHAP and example-based approaches such as counterfactual explanations.

Inherent interpretable models, are built-in explanations inherently from the model itself due to the models' simple structures, including decision sets~\citet{lakkaraju2016interpretable} or generalized linear models \chenhao{add reference here?}\shi{see WOE paper}. 
For deep learning models, built-in explanations may also be derived from specific architecture such as attention in NLP.
These explanations are directly derived from $g$.

Typical feature-based explanations include LIME~\citet{ribeiro2016should}, SHAP~\citet{lundberg2017unified}, and gradient-based methods \chenhao{add references}.
Gradient-based methods use gradients from $g$ to generate explanations. 
Both LIME and SHAP use local surrogate models to compute importance scores. The local surrogate model is trained based on $g$. 
Alternatively, counterfactual explanations provide hypothetical examples with minimal changes to the original feature values that would result in a different pre-defined output, in other words, counterfactual explanations provide ``what-if'' instances for a different model outcome.
That is, counterfactual explanations are also derived from the \decisionboundary, $g$.


All in all, current machine explanations are based on the model's decision boundary conditioned on a model, without taking into account of the task boundary or the error boundary. 
Hence, $E$ is bounded by $g$. 
Although we are not exhaustive in discussing all approaches to explaining machine predictions, we believe that for a wide variety of commonly-used explanation methods, it holds that machine explanations are derived from $g$.
We will center the discussion in this section on such explanations and mention a couple of exceptions in \secref{sec:explanation_challenges}.

\begin{figure}
    \centering
     \includegraphics[width=.45\columnwidth]{figs/explanation.jpeg}
    \caption{The limited effect of explanations without any human intuition.}
    \label{fig:explanation_local}
\end{figure}

\paragraph{Situating current explanations in our theoretical framework.}
To integrate the above discussion in our our causal diagrams, $E$ is directly derived from the machine learning models $g$, to provide additional information related to the prediction $\hat{Y}$. 
To simplify the discussion, we focus on the local setting for discovery tasks when $\hat{Y}$ is shown.

The key insight is that machine explanation $E$ is independent of $Y$ and $\error$ conditioned on $g$.
{\bf If we do not make any extra assumptions, humans cannot extract any information from $E$ beyond the model, therefore, it is impossible to achieve complementary performance simply by showing machine explanations.}

As a concrete example, consider the case of prostate cancer diagnosis with an alien who has never seen human body (i.e., guaranteeing that there is no intuition about this task).
\chenhao{I think that the deceptive review is also in this category, but I will keep the prostate cancer case for now.}
This extra explanation, either by highlighting the area that the model pays attention to or showing colored saliency maps to indicate the mechanism behind the model, cannot provide any meaningful information to the decision maker, i.e., the alien.

As we discussed in \secref{sec:digrams}, one way that we can improve human understanding of the task boundary ($\humany$) is through $\humanu$, by improving human understanding of the error boundary.
However, this cannot be achieved without extra assumptions about human intuitions either because humans cannot extract anything from $E$ beyond $g$.
Next, we discuss how explanations can be integrated with human explanations to achieve an improved understanding.


Explanations can certainly improve human understanding of the \decisionboundary.
In the case of emulation tasks, this is sufficient for inferring the \errorboundary for the sake of debugging because humans understand the \taskboundary.
Note that human understanding of the \taskboundary is a big assumption about human intuitions.
Next, we discuss how human intuitions can help in discovery tasks.


\subsection{Explanations + Human Intuitions}

In order to improve human understanding of the \taskboundary and the \errorboundary beyond the capability of model predictions, we need to make assumptions about human intuitions.
Human intuitions broadly refer to any (partial) knowledge that humans may have about \taskboundary, \decisionboundary, and \errorboundary.
We discuss two possible ways that such an improved understanding can be achieved.

\paragraph{Providing information for existing human intuitions.}
One possible way that human intuitions can help humans leverage explanations is to allow them to use their partial knowledge about the \taskboundary, althoguh this knowledge is likely not sufficient to perfectly determine the correct label.
Such partial knowledge can be used together with explanations to improve human understanding of the \errorboundary and then the \taskboundary (see \figref{fig:explanation_human}).
We categorize human intuitions into two groups: 1) {\em relevance}, whether a feature is relevant to the \taskboundary and 2) {\em mechanism}, how a feature is associated with the \taskboundary (e.g., positively or negatively correlated).

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/exp_human.jpg}
        \caption{Integrating with existing human intuitions.}
        \label{fig:explanation_human}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/exp_expand.jpg}
        \caption{Expanding human intuitions.}
        \label{fig:explanation_expand}
    \end{subfigure}
    \caption{Explanations can provide effective support in combination with human intuitions.}
\end{figure}

\begin{itemize}
    \item Humans can tell that the model is using irrelevant information.
    In the example of prostate cancer diagnosis, if the explanation points to an area outside the prostate, then the decision maker, who knows where the prostate is in the image, can realize that the model prediction is based on wrong evidence.
    \chenhao{a figured could help; deceptive review can work too, but may be it is good to have two examples; we can discuss this.}
    Note that in practice, irrelevant evidence does not entail wrong predictions for the model.
    Thus, another important premise for this assumption to result in complementary performance lies in that wrong evidence has strong correlation with wrong predictions, an important empirical hypothesis that one needs to validate.
    \item Humans can tell that the model is using a wrong mechanism.
    Continuing with the example of prostate cancer diagnosis, the explanations can show that the model predicts cancer because the dark area in region A  is associated with positive diagnosis.
    The decision maker instead knows that in general, dark areas in that region should be negatively associated with cancer diagnosis, and then they can decide that the model prediction is wrong.  
\end{itemize}


\paragraph{Expanding human intuitions.}
Another way that explanations can improve human understanding is by expanding human intuitions (see \figref{fig:explanation_expand}).
Consider the example of ``chicago'' as an important indicator for deceptive review detection.
The reason that ``chicago'' is reliably associated with deceptive reviews in this dataset are for two reasons:
1) people are less likely to provide specific details when they write fictional texts (theory I);
2) deceptive reviews in this dataset are written by crowdworkers on mechanical turk for hotels in Chicago (fact II).
So one possible way that explanations can expand human intuitions if they can derive the above theory I.
This can lead to complementary performance, especially for out-of-distribution examples such as reviews in New York City.
Then, human decision makers can apply this intuition, but the model cannot.
Similarly, in the extreme example of alien performing prostate cancer diagnosis, this is a possible way that explanations can help is that aliens acquire reliable associations, although it seems unlikely that aliens can exceed model performance in this case.
Formally, this key update for this scenario likes in $E$ influence human intuitions in the next time step $\mathcal{H}^{t+1}$.




\subsection{Towards Effective Explanations for Improving Human Understanding}
\label{sec:explanation_challenges}

Our analyses identify future directions towards building effective explanations for improving human understanding.

\paragraph{Generating explanations.}
First, our work highlights 
that an important direction towards effective explanations is to take into account human intuitions when generating machine explanations.
In many ways, this already happens:

\begin{itemize}
    \item We do not present all the parameters in a neural network because we assume that humans cannot understand these parameters.
    \item We avoid red and green colors because we assume that color-blind people fail to extract meaningful information from indistinguishable saliency map.\chacha{sounds like a design choce but not depend on explanation methods, maybe i misunderstand}
    \item We choose hyper-parameter because empirical evidence shows that gradients from this layer matches human perception best. \chenhao{shi, can you find a ference for this and update the wording to be more precise?}
\end{itemize}

However, these generic human intuitions are insufficient for improving human understanding of the \taskboundary and the \errorboundary.
It is important to think about how machine explanations can be tailored to either leveraging existing human knowledge or expanding human intuitions, or other ways that human intuitions can work together with explanations.
Another important ingredient for this direction is the ability to measure human intuitions.

Another direction is to incorporate $f$ and $u$ into explanations. 
An important premise for explanations working together with human intuitions lies in that machine explanations capture the mechanism or the relevance underlying the model.
Indeed, faithfulness receives significant interest from the machine learning community in the perspective of explaining the mechanisms behind a model.
However, faithfulness to $g$ alone is insufficient to improving human understanding of the \taskboundary and the \errorboundary.


In order to effectively improve human understanding of $f$ and $u$, it would be useful to explicitly incorporate $f$ and $u$ into the generation process of $E$.
For example, a simple way to incorporate $u$ is to report the error rate in a development set. 
In the case of deceptive review detection, it could be when ``Chicago'' is used as an important feature, the model is 90\% accurate.
This allows humans to have access to part of the error boundary and have a more accurate $\humanu$.
Again, in order for such explanations to succeed, two conditions need to be satisfied: 1) such explanations are ``faithful'' (i.e., the model is indeed 90\% accurate when ``Chicago'' is used);
2) humans can interpret 90\% and act accordingly, which pertains to the research on numeracy.



\paragraph{Articulating and measuring human intuitions.} Our framework highlights the importance of human intuitions in leveraging machine explanations.
Implicit in the hypothesis that machine explanations can improve human understanding are assumptions about human intuitions.
First, we need to make these assumptions about human intuitions explicit so that the research community can collectively study them rather than repeating trial-and-error on the effect of explanations on an end outcome such as task accuracy.
We recommend the research community be precise about what machine explanations are trying to achieve and what type of human intuitions is required to achieve success with machine explanations.

Second,  to make progress in experimental studies with machine explanations, we need to develop ways to either control or measure human intuitions.
This can be very challenging in practice.
To illustrate a simple case study on this example, we will present an experiment where we control human intuitions in human-AI decision making.


To summarize, we emphasize the following three takeaways.

\begin{itemize}
    \item Current machine explanations are mainly about the model and its utility for human understanding of the \taskboundary and the \errorboundary is thus limited by the model.
    \item Human intuitions are a critical component to realize the promise of machine explanations in improving human understanding and achieving complementary performance.
    \item We need to articulate our assumptions about human intuitions and take steps towards validating and measuring human intuitions, and incorporate human intuitions, $f$, and $u$ into the generation of machine explanations.
\end{itemize}









==> explanation_role.tex <==

\subsection{Explanation Role in the Theoretical Framework}

\chenhao{should we start from random explanations?}


\para{Discovery.}

Figure 7a:

1) case 1: in loan application, showing the annual income of the person is the most important positive related factor help human understand $\hat{Y}^H$ as positive and then because $E$ explain a reasonable mechanism so $U^H$ as 1, thus given both $U^H$ and $\hat{Y}^H$, $Y^H$ as positive.
\chenhao{I do not understand this ... it seems that this is still $U^H$ first.}

2) case 2: in loan application, showing gender as the most important feature related to a positive prediction makes human doubt the machine prediction, thus they may guess $U^H$ as zero (incorrect), which leads to $\hat{Y}$ as positive (because positive related feature is more than negative related feature given $E$). Finally, both 
\chacha{not a good example}

3) $E$ provide nothing to $U^H$, $\hat{Y}^H$, or $Y^H$. However, human guesses of the $Y$ and $Y^H$ determines $U^H$.

Figure 7b:

1) case 1: in loan application, showing a positive label associated with the most important feature as annual income (signed feature weights) helps $Y^H$, and thus $U^H$.

2) case 2: in loan application, showing a negative label associated with the most important feature as gender (signed feature wights) makes people doubt $U^H$. \chacha{but even in this case $U^H$ can be arbitrarily 1 or 0 hence doesnt help $Y^H$, in other words, machine makes prediction based on wrong feature doesn't help people to judge the true label. So there are no case 2 figures in both 7a and 7b}.

3) $E$ doesn't help.


Examples to think about:

cancer diagnosis (vision)

loan application (tabular)

cat vs. dog image classification







\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{figs/discovery_exp_E.png}\\
    \includegraphics[width=.8\columnwidth]{figs/discovery_exp_E_Y.png}
    \caption{$E$ in discovery tasks}
    \label{fig:discovery_E}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{figs/emulation_exp_1.png}
    \caption{$E$ in emulation tasks}
    \label{fig:emulation_E}
\end{figure}


In order to illustrate how $E$ affects causal paths, we use two examples: prostate cancer diagnosis (image data) and loan application (tabular data). 

\para{Emulation.}
For emulation tasks, we use cat vs. dog image classification as the pivot example illustrate how $E$ affects different causal paths. 
Human has perfect understanding of the task. 
There are multiple possible paths. As shown in \figref{fig:emulation_E:} (a), we draw all the possible arrows, which we call as the complete graph. However, those arrows do not necessary exist in the human-AI interaction. We show 2 other possible cases:
1) $E$ leads to human guesses of $\hat{Y}$, and then both $\hat{Y}$ and $Y/Y^H$ lead to $U^H$. For example, $E$ highlight an area of the cat whisker, human then guess $\hat{Y^H}$ is cat, which is aligned with groundtruth label $Y$. Then $U^H$ must be 1.
2) $E$ does not help anything. In this case, $E$ could be evidence, which does not lead to any human understanding of the $U$ or $\hat{Y}$.











\subsection{Takeaways}

Machine explanations are incomplete


identify what people hope to achieve via explanations

whether mechanism wrong or is mechanism doesn't help

Mechanisms of explanations: how can they help? current they mainly help in conveying information about $g$
Explanations can affect which path is dominant.
Explanations that help one measure might not help the other
(unfaithful explanations can be misleading?) Example 1: highlighting prostate region helps non-expert even if the model is trained with the labels flipped

uncertainty?

==> generalized_definition.tex <==
\section{Generalized Definitions} 

We extend the above framework to account for tasks beyond 
binary
classification tasks.
For multi-class classification and regression tasks, $g$ and $f$ cannot be represented by a hyper-surface that partitions the data into two sets.
We refer to the corresponding concepts as {\em decision curves} and {\em task curves}.

The downstream task's notion of error can be fine-grained, i.e., not all errors are equally bad.
In particular, false positives and false negatives can result in different utilities.
For instance, false positives can lead to substantial harm to individuals and the society in recidivism prediction (i.e., unnecessary time in jail), while false negatives may be more detrimental in surveillance testing during the pandemic (e.g., missing a positive COVID-19 case).
In this case, we generalize the definition of error boundary to {\em utility curves}:
We use a utility value to measure the utility of a (in)correct prediction $I(h(x)=f(x))$.
We can still use the same notation, $u(\cdot)$, to denote the utility function,
but the target domain can be more general than $\{1, 0\}$.
We refer to this generalized notion as {\em utility curves}.


For instance, utility curves naturally capture diverse preferences in regression tasks. \chacha{but utility curve is not for the sake of regression task, am i understanding correctly? false positve and false negative can also be different in classification}
If the ground-truth price of a house is $300,000$, the predictions of $280,000$ and $350,000$ are both wrong, but one might prefer the $280,000$ prediction if you want to be closer to actual value; another person might prefer the $350,000$ prediction if you prefer not to underestimate. 


We focus on classification tasks in this work and thus discuss decision boundary, task boundary, and error boundary in the rest of the paper. 
Our main claims can be easily generalized to task curves, decision curves, and utility curves, and we leave experimental studies on these generalized studies to future work.\shi{if the discussion that follows this goes back to classification, maybe we should talk about generalization and caveats afterwards?}
\chenhao{yeah, this should be at the end of 2.1}

We further distinguish the understanding of a concept by an agent with superscripts.
For example, $f^h$ refers to human understanding of the task boundary, and $f^{h+m}$ refers to human understanding of the task boundary with machine assistance.
We use a binary classification task ($Y = \{0, 1\}$) to illustrate our definitions and then provide generalized definitions for more complex scenarios. 
We then show that these three boundaries provide critical dimensions for capturing any understanding with respect to the task/model.

==> global_understanding.tex <==
\section{Global understanding}
\label{sec:global_understanding}


\subsection{}

teaching effect / time dimension / updates in humans


\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{figs/global.png}
    \caption{\chacha{change $f$ to $H$}}
    \label{fig:my_label}
\end{figure}



1. introducing human initial intuitions $H_0$
2. explain how $H_0$ updates over time (each interaction)
3. local vs global

updates only happen if human received feedback








==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> measuring_understanding.tex <==
\section{Three Core Concepts for Measuring Human Understanding}
\label{sec:human_understanding}

\begingroup
\setlength{\intextsep}{1pt}%

\begin{wrapfigure}{r}{0.44\textwidth}
        \centering
        \includegraphics[width=.4\textwidth]{figs/decision_error_v2.pdf}
        \caption{
        Illustration of three core concepts.
        }
        \label{fig:decision_error}
\end{wrapfigure}

We identify three core concepts of interest in human-AI decision making \rev{in classification tasks}: \taskboundary, \decisionboundary, and \errorboundary.
We present high-level definitions of these concepts here and then formalize them in \secref{sec:framework}.\footnote{
In this work, we omit subjective measures.}
We use a two-dimensional binary classification problem to 
illustrate the three concepts of interest (\figref{fig:decision_error}).
{\em \Taskboundary} (dashed line)
defines the mapping from inputs to ground-truth labels: inputs on the left are positive and the ones on the right are negative.
{\em \Decisionboundary} (solid line)
determines model predictions.
Consequently, 
The yellow highlighted area between the two boundaries captures {\em \errorboundary}, i.e., where the model prediction is incorrect.
With a perfect model, the \decisionboundary would be an exact match of the \taskboundary, and \errorboundary never happens.



To the best of our knowledge, \rev{most} existing quantitative behavioral measures of human understanding map to one of these three concepts.
Building on a recent survey \citep{lai2021towards}, we identify \rev{31} papers \rev{with two criteria:} 1) use ML models and explanations with the goal of improving human understanding and 2) conduct empirical human studies to evaluate human understanding with quantitative metrics.
The three concepts allow us to \rev{group} existing works into \rev{different} categories (see Appendix \secref{sec:paper_summary}).

\endgroup


